DeLiRa: Self-Supervised Depth, Light, and Radiance Fields

Differentiable volumetric rendering is a powerful paradigm for 3D reconstruction and novel view synthesis. However, standard volume rendering approaches struggle with degenerate geometries in the case of limited viewpoint diversity, a common scenario in robotics applications. In this work, we propose to use the multi-view photometric objective from the self-supervised depth estimation literature as a geometric regularizer for volumetric rendering, significantly improving novel view synthesis without requiring additional information. Building upon this insight, we explore the explicit modeling of scene geometry using a generalist Transformer, jointly learning a radiance field as well as depth and light fields with a set of shared latent codes. We demonstrate that sharing geometric information across tasks is mutually beneficial, leading to improvements over single-task learning without an increase in network complexity. Our DeLiRa architecture achieves state-of-the-art results on the ScanNet benchmark, enabling high quality volumetric rendering as well as real-time novel view and depth synthesis in the limited viewpoint diversity setting.

==> equations.tex <==


% \begin{equation}
% K = 
% \begin{bmatrix}
% f_w &  0  & c_w \\
%  0  & f_h & c_h \\
%  0  &  0  &  1  \\
% \end{bmatrix}
% \end{equation}


% We assume input images of $H \times W$ resolution. Our sampling procedure is governed by vertical and horizontal stride parameters $s_h$ and $s_w$. Because these parameters are fixed, we instead randomly select sampling offsets $o_h \in [0,s_h]$ and $o_w \in [0,s_w]$ (Figure \ref{fig:grid_sampling}).

% \begin{equation}
% \textbf{T}_t = 
% \begin{bmatrix}
% \textbf{R}_t & \textbf{t}_t \\
% \textbf{0} & 1  \\
% \end{bmatrix}
% \end{equation}

% \begin{equation}
%     \textbf{t}_t = (x,y,z)_t
% \end{equation}


% \begin{equation}
% \begin{bmatrix}
% (r,g,b,\sigma)_1 \\
% \vdots \\
% (r,g,b,\sigma)_k \\
% \vdots \\
% (r,g,b,\sigma)_K \\
% \end{bmatrix}_{ij}
% \end{equation}


==> figures/grid_sampling.tex <==

\begin{figure}[t!]
\centering
\includegraphics[width=0.45\textwidth]{images/grid_sampling.png}
\caption{
\textbf{Example of grid sampling}, with $s_w=s_h=3$, $o_w = 1$, and $o_h = 2$. In this case, a $6 \times 8$ image is downsampled to $2 \times 3$.
}
\label{fig:grid_sampling}
\vspace{-4mm}
\end{figure}


==> figures/photo.tex <==

\begin{figure}[t!]
\centering
\subfloat[Target RGB]{
\includegraphics[width=0.11\textwidth]{images/photo/rgb0.png}}
\subfloat[Vol. depth]{
\includegraphics[width=0.11\textwidth]{images/photo/depth.png}}
% \\
\subfloat[Warped context]{
\includegraphics[width=0.11\textwidth]{images/photo/warped.png}}
\subfloat[Photo. loss]{
\includegraphics[width=0.11\textwidth]{images/photo/photo.png}}
\caption{
\textbf{Example of the multi-view photometric objective} used as additional self-supervision for volumetric rendering. 
}
\label{fig:photo}
\vspace{-2mm}
\end{figure}


==> figures/results.tex <==

\begin{figure*}[t!]
\centering
\subfloat{
\includegraphics[width=0.18\textwidth,height=1.6cm]{
images/qualitative/0/rgb_gt.png}}
\subfloat{
\includegraphics[width=0.18\textwidth,height=1.6cm]{
images/qualitative/0/nerf_vol_rgb.png}}
\subfloat{
\includegraphics[width=0.18\textwidth,height=1.6cm]{
images/blank.png}}
\subfloat{
\includegraphics[width=0.18\textwidth,height=1.6cm]{
images/qualitative/0/nerfine_vol_rgb.png}}
\subfloat{
\includegraphics[width=0.18\textwidth,height=1.6cm]{
images/qualitative/0/nerfine_single_rgb.png}}
\\
\setcounter{subfigure}{0}
\subfloat{
\includegraphics[width=0.18\textwidth,height=1.6cm]{
images/qualitative/0/depth_gt.png}}
\subfloat{
\includegraphics[width=0.18\textwidth,height=1.6cm]{
images/qualitative/0/nerf_vol_depth.png}}
\subfloat{
\includegraphics[width=0.18\textwidth,height=1.6cm]{
images/qualitative/0/mono_depth.png}}
\subfloat{
\includegraphics[width=0.18\textwidth,height=1.6cm]{
images/qualitative/0/nerfine_vol_depth.png}}
\subfloat{
\includegraphics[width=0.18\textwidth,height=1.6cm]{
images/qualitative/0/nerfine_single_depth.png}}
\\
\vspace{2mm}
\subfloat{
\includegraphics[width=0.18\textwidth,height=1.6cm]{
images/qualitative/1/rgb_gt.png}}
\subfloat{
\includegraphics[width=0.18\textwidth,height=1.6cm]{
images/qualitative/1/nerf_vol_rgb.png}}
\subfloat{
\includegraphics[width=0.18\textwidth,height=1.6cm]{
images/blank.png}}
\subfloat{
\includegraphics[width=0.18\textwidth,height=1.6cm]{
images/qualitative/1/nerfine_vol_rgb.png}}
\subfloat{
\includegraphics[width=0.18\textwidth,height=1.6cm]{
images/qualitative/1/nerfine_single_rgb.png}}
\\
\setcounter{subfigure}{0}
\subfloat[Ground-truth]{
\includegraphics[width=0.18\textwidth,height=1.6cm]{
images/qualitative/1/depth_gt.png}}
\subfloat[Baseline (w/o self-sup.)]{
\includegraphics[width=0.18\textwidth,height=1.6cm]{
images/qualitative/1/nerf_vol_depth.png}}
\subfloat[Monodepth (self-sup.)]{
\includegraphics[width=0.18\textwidth,height=1.6cm]{
images/qualitative/1/mono_depth.png}}
\subfloat[Volumetric Rendering]{
\includegraphics[width=0.18\textwidth,height=1.6cm]{
images/qualitative/1/nerfine_vol_depth.png}}
\subfloat[Light and Depth Fields]{
\includegraphics[width=0.18\textwidth,height=1.6cm]{
images/qualitative/1/nerfine_single_depth.png}}
\caption{
\textbf{Qualitative results for depth and view synthesis} of our method, considering different decoding strategies. 
%\VS{Figure missing row labels.}
}
\label{fig:results}
\vspace{-2mm}
\end{figure*}




% \begin{figure*}[t!]
% \centering
% %
% \subfloat{
% \includegraphics[width=0.18\textwidth,height=1.6cm]{
% images/qualitative/0/rgb_gt.png}}
% \subfloat{
% \includegraphics[width=0.18\textwidth,height=1.6cm]{
% images/qualitative/0/nerf_vol_rgb.png}}
% \subfloat{
% \includegraphics[width=0.18\textwidth,height=1.6cm]{
% images/blank.png}}
% \subfloat{
% \includegraphics[width=0.18\textwidth,height=1.6cm]{
% images/qualitative/0/nerfine_vol_rgb.png}}
% \subfloat{
% \includegraphics[width=0.18\textwidth,height=1.6cm]{
% images/qualitative/0/nerfine_single_rgb.png}}
% % \subfloat{
% % \includegraphics[width=0.18\textwidth,height=1.6cm]{
% % images/qualitative/0/nerfine_refine_rgb.png}}
% \\
% \setcounter{subfigure}{0}
% \subfloat{
% \includegraphics[width=0.18\textwidth,height=1.6cm]{
% images/qualitative/0/depth_gt.png}}
% \subfloat{
% \includegraphics[width=0.18\textwidth,height=1.6cm]{
% images/qualitative/0/nerf_vol_depth.png}}
% \subfloat{
% \includegraphics[width=0.18\textwidth,height=1.6cm]{
% images/qualitative/0/mono_depth.png}}
% \subfloat{
% \includegraphics[width=0.18\textwidth,height=1.6cm]{
% images/qualitative/0/nerfine_vol_depth.png}}
% \subfloat{
% \includegraphics[width=0.18\textwidth,height=1.6cm]{
% images/qualitative/0/nerfine_single_depth.png}}
% % \subfloat{
% % \includegraphics[width=0.18\textwidth,height=1.6cm]{
% % images/qualitative/0/nerfine_refine_depth.png}}
% \\
% \vspace{2mm}
% %
% \subfloat{
% \includegraphics[width=0.18\textwidth,height=1.6cm]{
% images/qualitative/1/rgb_gt.png}}
% \subfloat{
% \includegraphics[width=0.18\textwidth,height=1.6cm]{
% images/qualitative/1/nerf_vol_rgb.png}}
% \subfloat{
% \includegraphics[width=0.18\textwidth,height=1.6cm]{
% images/blank.png}}
% \subfloat{
% \includegraphics[width=0.18\textwidth,height=1.6cm]{
% images/qualitative/1/nerfine_vol_rgb.png}}
% \subfloat{
% \includegraphics[width=0.18\textwidth,height=1.6cm]{
% images/qualitative/1/nerfine_single_rgb.png}}
% % \subfloat{
% % \includegraphics[width=0.18\textwidth,height=1.6cm]{
% % images/qualitative/1/nerfine_refine_rgb.png}}
% \\
% \setcounter{subfigure}{0}
% \subfloat[Ground-truth]{
% \includegraphics[width=0.18\textwidth,height=1.6cm]{
% images/qualitative/1/depth_gt.png}}
% \subfloat[Baseline (w/o self-sup.)]{
% \includegraphics[width=0.18\textwidth,height=1.6cm]{
% images/qualitative/1/nerf_vol_depth.png}}
% \subfloat[Monodepth (self-sup.)]{
% \includegraphics[width=0.18\textwidth,height=1.6cm]{
% images/qualitative/1/mono_depth.png}}
% \subfloat[Volumetric Rendering]{
% \includegraphics[width=0.18\textwidth,height=1.6cm]{
% images/qualitative/1/nerfine_vol_depth.png}}
% \subfloat[Light and Depth Fields]{
% \includegraphics[width=0.18\textwidth,height=1.6cm]{
% images/qualitative/1/nerfine_single_depth.png}}
% % \subfloat[Refined (V)]{
% % \includegraphics[width=0.18\textwidth,height=1.6cm]{
% % images/qualitative/1/nerfine_refine_depth.png}}
% %
% \caption{
% \textbf{Qualitative results for depth and view synthesis} of our method, considering different decoding strategies. 
% }
% \label{fig:results}
% \vspace{-2mm}
% \end{figure*}

% % \begin{figure*}[t!]
% % \centering
% % \subfloat[RGB]{
% % \includegraphics[width=0.13\textwidth]{images/results/nmvs_gt_rgb_0.png}}
% % \subfloat[NeRF RGB]{
% % \includegraphics[width=0.13\textwidth]{images/results/nmvs_nerfine_rgb_0.png}}
% % \subfloat[NeRFiNe RGB]{
% % \includegraphics[width=0.13\textwidth]{images/results/nmvs_nerfine_rgb_0.png}}
% % \subfloat[Depth]{
% % \includegraphics[width=0.13\textwidth]{images/results/nmvs_gt_depth_0.png}}
% % \subfloat[NeRF depth]{
% % \includegraphics[width=0.13\textwidth]{images/results/nmvs_monodepth_depth_0.png}}
% % \subfloat[Monodepth depth]{
% % \includegraphics[width=0.13\textwidth]{images/results/nmvs_monodepth_depth_0.png}}
% % \subfloat[NeRFiNe depth]{
% % \includegraphics[width=0.13\textwidth]{images/results/nmvs_nerfine_depth_0.png}}
% % \caption{
% % }
% % \label{fig:results}
% % \end{figure*}


==> figures/smaller.tex <==


\begin{figure}[t!]
\centering
\subfloat{
\includegraphics[width=0.45\textwidth,trim={1.1cm 0.4cm 1.3cm 1.1cm},clip]{images/plots/num_lat_vec.pdf}}
\\
% \hspace{-2mm}
% \vspace{-2mm}
\subfloat{
\includegraphics[width=0.45\textwidth,trim={1.1cm 0.4cm 1.3cm 1.1cm},clip]{images/plots/dim_lat_vec.pdf}}
\vspace{-3mm}
\caption{
\textbf{Depth and view synthesis performance} on \emph{ScanNet} (\emph{scene0653}), with varying latent space shapes. 
}
\label{fig:smaller}
\end{figure}


% \begin{figure}[t!]
% \centering
% \subfloat{
% \includegraphics[width=0.23\textwidth,trim={1.1cm 0.4cm 1.3cm 1.1cm},clip]{images/plots/num_lat_vec.pdf}}
% % \\
% % \hspace{-2mm}
% % \vspace{-2mm}
% \subfloat{
% \includegraphics[width=0.23\textwidth,trim={1.1cm 0.4cm 1.3cm 1.1cm},clip]{images/plots/dim_lat_vec.pdf}}
% \vspace{-3mm}
% \caption{
% \textbf{Depth and view synthesis performance} on \emph{ScanNet} (\emph{scene0653}), with varying latent space shapes. 
% }
% \label{fig:smaller}
% \end{figure}


==> tables/nmvs_generalization.tex <==
\captionsetup[table]{skip=6pt}

\begin{table*}[t!]
\small
\renewcommand{\arraystretch}{1.1}
\centering
{
\setlength{\tabcolsep}{0.3em}
\begin{tabular}{l|c|c||c|c|c|c||c|c}
\toprule
\multirow{2}[2]{*}{\textbf{Method}} & 
\multirow{2}[2]{*}{\rotatebox{90}{\scriptsize{Shared}}} & 
\multirow{2}[2]{*}{\rotatebox{90}{\scriptsize{Decoder}}} & 
\multicolumn{4}{c||}{\textbf{Depth}} &
\multicolumn{2}{c}{\textbf{View Synthesis}}
\\
\cmidrule(lr){4-7} \cmidrule(lr){8-9} 
\renewcommand{\arraystretch}{1.0}
& & &
Abs.Rel.$\downarrow$ &
Sq.Rel.$\downarrow$ &
RMSE$\downarrow$ &
$\delta < {1.25}$$\uparrow$ &
PSNR$\uparrow$ & 
SSIM$\uparrow$
\\
\midrule
& & \scriptsize{R}  
& 0.055 & 0.014 & 0.131 & 0.970 & 28.892 & 0.932
\\
& \multirow{-2}{*}{---} & \scriptsize{DL}  
& 0.054 & 0.028 & 0.138 & 0.966 & 28.967 & 0.929 
\\
\cmidrule{2-9}
& & \scriptsize{R}
& 0.057 & 0.017 & 0.143 & 0.964 & 27.563 & 0.906 
\\
& \multirow{-2}{*}{Dec} & \scriptsize{DL}  
& 0.060 & 0.034 & 0.147 & 0.961 & 26.484 & 0.889 
\\
\cmidrule{2-9}
& & \scriptsize{R}  
& 0.061 & 0.022 & 0.152 & 0.953 & 27.162 & 0.891 
\\
& \multirow{-2}{*}{Lat} & \scriptsize{DL} 
& 0.063 & 0.041 & 0.155 & 0.949 & 25.892 & 0.872 
\\
\cmidrule{2-9}
& & \scriptsize{R}
& 0.486 & 0.672 & 1.207 & 0.455 & 14.231 & 0.342 
\\
\multirow{-9}{*}{\Acronym} 
& \multirow{-2}{*}{All} & \scriptsize{DL}  
& 0.479 & 0.681 & 1.198 & 0.449 & 13.989 & 0.350 
\\
\bottomrule
\end{tabular}
}
\caption{
\textbf{Multi-scene depth estimation and novel view synthesis results}, on \emph{ScanNet-Frontal}. The \emph{shared} column, \emph{Dec} denotes a single shared decoder with per-scene latent spaces, \emph{Lat} denotes a single shared latent space with per-scene decoders, and \emph{All} denotes sharing both the latent space and the decoder. Interestingly, we notice marginal degradation in performance when using scene-specific latent spaces with a single shared decoder. Using a shared latent space, with scene-specific decoders, leads to further degradation in performance. Moreover, depth estimation is more robust to multi-scene generalization than view synthesis, since geometry is more transferable across scenes. 
}
\label{table:nmvs_generalization}
\end{table*}





% \captionsetup[table]{skip=6pt}

% \begin{table*}[t!]
% \small
% \renewcommand{\arraystretch}{0.95}
% \centering
% {
% \small
% \setlength{\tabcolsep}{0.3em}
% \begin{tabular}{l|c|c|c|c||c|c|c|c||c|c}
% \toprule
% \multirow{2}[2]{*}{\textbf{Version}} & 
% \multirow{2}[2]{*}{\rotatebox{90}{\scriptsize{Self-Sup.}}} & \multirow{2}[2]{*}{\rotatebox{90}{\scriptsize{Shared}}} & \multirow{2}[2]{*}{\rotatebox{90}{\scriptsize{Decoder}}} & \multirow{2}[2]{*}{\rotatebox{90}{\scriptsize{\# Queries}}} & \multicolumn{4}{c||}{\textbf{Depth}} &
% \multicolumn{2}{c}{\textbf{View Synthesis}}
% \\
% \cmidrule(lr){6-9} \cmidrule(lr){10-11} 
% \renewcommand{\arraystretch}{1.0}
% & & & & &
% Abs.Rel.$\downarrow$ &
% Sq.Rel.$\downarrow$ &
% RMSE$\downarrow$ &
% $\delta < {1.25}$$\uparrow$ &
% PSNR$\uparrow$ & 
% SSIM$\uparrow$
% \\
% %
% \midrule
% \rowcolor{Gray}
% Volumetric & \checkmark & & V & $128$  
% & 0.056 & 0.017 & 0.134 & 0.966 & 28.671 & 0.912 
% \\
% & & & V & $128$  
% & 0.054 & 0.014 & 0.131 & 0.971 & 29.279 & 0.927 
% \\
% % \multirow{-2}{*}{Distilled (V $\shortrightarrow$ LD)} 
% & \multirow{-3}{*}{\checkmark} & & LD & $1$  
% % & 0.055 & 0.029 & 0.129 & 0.970 & 26.312 & 0.881 \\
% & 0.057 & 0.029 & 0.139 & 0.962 & 27.663 & 0.901
% % \\
% % \rowcolor{Gray}
% % & & & LD & $1$  
% % % & 0.055 & 0.027 & 0.128 & 0.969 & 26.434 & 0.883 \\
% % & 0.054 & 0.027 & 0.137 & 0.964 & 27.934 & 0.904 
% \\
% % \rowcolor{Gray}
% % \multirow{-3}{*}{Refined (LD $\shortrightarrow$ V)} 
% \multirow{-3}{*}{Distilled} 
% & \multirow{-2}{*}{\checkmark} & & DL & $1\!\!+\!\!16$  
% % & 0.054 & 0.029 & 0.127 & 0.971 & 29.331 & 0.912 \\
% & 0.055 & 0.025 & 0.132 & 0.967 & 29.073 & 0.910 
% \\
% %
% \midrule
% \rowcolor{Gray}
% Volumetric & \checkmark & L & V & $128$  
% & 0.059 & 0.018 & 0.145 & 0.956 & 28.448 & 0.904 
% \\
% & & & V & $128$  
% & -.---- & -.---- & -.---- & -.---- & -.---- & -.---- 
% \\
% \multirow{-2}{*}{Distilled (V $\shortrightarrow$ LD)} 
% & \multirow{-2}{*}{\checkmark} & \multirow{-2}{*}{L} & LD & $1$  
% & -.---- & -.---- & -.---- & -.---- & -.---- & -.---- 
% \\
% \rowcolor{Gray}
% & & & LD & $1$  
% & -.---- & -.---- & -.---- & -.---- & -.---- & -.---- 
% \\
% \rowcolor{Gray}
% \multirow{-2}{*}{Guided (LD $\shortrightarrow$ V)} 
% & \multirow{-2}{*}{\checkmark} & \multirow{-2}{*}{L} & LD+V & $1\!\!+\!\!16$  
% & -.---- & -.---- & -.---- & -.---- & -.---- & -.---- 
% \\
% %
% \midrule
% \rowcolor{Gray}
% Volumetric & \checkmark & D & V & $128$  
% & 0.057 & 0.016 & 0.143 & 0.962 & 29.188 & 0.914 
% \\
% \rowcolor{White}
% & & & V & $128$  
% & 0.056 & 0.017 & 0.141 & 0.964 & 29.043 & 0.906 
% \\
% \multirow{-2}{*}{Distilled (V $\shortrightarrow$ LD)} 
% & \multirow{-2}{*}{\checkmark} & \multirow{-2}{*}{D} & LD & $1$  
% % & 0.055 & 0.034 & 0.138 & 0.968 & 26.084 & 0.879 \\
% & 0.060 & 0.034 & 0.143 & 0.961 & 26.084 & 0.879 
% \\
% \rowcolor{Gray}
% Distilled (V $\shortrightarrow$ LD, frozen)
% & \checkmark & D & LD & $1$  
% % & 0.055 & 0.028 & 0.135 & 0.968 & 26.101 & 0.880 \\
% & 0.062 & 0.041 & 0.147 & 0.957 & 25.218 & 0.839 
% \\
% \rowcolor{White}
% & & & LD & $1$  
% % & 0.055 & 0.028 & 0.135 & 0.968 & 26.101 & 0.880 \\
% & 0.058 & 0.028 & 0.135 & 0.963 & 26.101 & 0.880 
% \\
% \rowcolor{White}
% \multirow{-2}{*}{Guided (LD $\shortrightarrow$ V)} 
% & \multirow{-2}{*}{\checkmark} & \multirow{-2}{*}{D} & LD+V & $1\!\!+\!\!16$  
% % & 0.055 & 0.031 & 0.133 & 0.969 & 28.355 & 0.905 \\
% & 0.057 & 0.026 & 0.136 & 0.964 & 28.565 & 0.905 
% \\
% \bottomrule
% \end{tabular}
% }
% \caption{
% \textbf{Multi-scene depth and view synthesis results}, on \emph{ScanNet-Frontal}. The \emph{self-sup.} column denotes the use of the self-supervised photometric objective (\Section \ref{sec:photometric_loss}) as an additional source of regularization. In the \emph{shared} column, \emph{D} denotes a single shared decoder with per-scene latent spaces, and \emph{L} denotes a single shared latent space with per-scene decoders. In the \emph{decoder} column, \emph{V} denotes outputs from the volumetric head, and \emph{LD} denotes outputs from the light and depth field heads. The \emph{\# queries} column indicates the number of queries required for pixel rendering. 
% }
% \label{table:nmvs_ablation}
% % \vspace{-4mm}
% \end{table*}




% \captionsetup[table]{skip=6pt}

% \begin{table*}[t!]
% \small
% \renewcommand{\arraystretch}{0.95}
% \centering
% {
% \small
% \setlength{\tabcolsep}{0.3em}
% \begin{tabular}{l|c|c||c|c|c|c||c|c}
% \toprule
% \multirow{2}[2]{*}{\textbf{Version}} & 
% \multirow{2}[2]{*}{\rotatebox{90}{\scriptsize{Shared}}} & 
% \multirow{2}[2]{*}{\rotatebox{90}{\scriptsize{Decoder}}} & 
% \multicolumn{4}{c||}{\textbf{Depth}} &
% \multicolumn{2}{c}{\textbf{View Synthesis}}
% \\
% \cmidrule(lr){4-7} \cmidrule(lr){8-9} 
% \renewcommand{\arraystretch}{1.0}
% & & &
% Abs.Rel.$\downarrow$ &
% Sq.Rel.$\downarrow$ &
% RMSE$\downarrow$ &
% $\delta < {1.25}$$\uparrow$ &
% PSNR$\uparrow$ & 
% SSIM$\uparrow$
% \\
% \midrule
% & & \scriptsize{R}  
% & 0.055 & 0.014 & 0.131 & 0.970 & 28.892 & 0.932
% \\
% \multirow{-2}{*}{\Acronym} 
% & & \scriptsize{DL}  
% & 0.054 & 0.028 & 0.138 & 0.966 & 28.967 & 0.929 
% \\
% \midrule
% & & \scriptsize{R}  
% & 0.061 & 0.022 & 0.152 & 0.953 & 27.162 & 0.891 
% \\
% \multirow{-2}{*}{\Acronym} 
% & \multirow{-2}{*}{Lat} & \scriptsize{DL} 
% & 0.063 & 0.041 & 0.155 & 0.949 & 25.892 & 0.872 
% \\
% \midrule
% & & \scriptsize{R}
% & 0.057 & 0.017 & 0.143 & 0.964 & 27.563 & 0.906 
% \\
% \multirow{-2}{*}{\Acronym} 
% & \multirow{-2}{*}{Dec} & \scriptsize{DL}  
% & 0.060 & 0.034 & 0.147 & 0.961 & 26.484 & 0.889 
% \\
% \midrule
% & & \scriptsize{R}
% & 0.057 & 0.017 & 0.143 & 0.964 & 27.563 & 0.906 
% \\
% \multirow{-2}{*}{\Acronym} 
% & \multirow{-2}{*}{All} & \scriptsize{DL}  
% & 0.060 & 0.034 & 0.147 & 0.961 & 26.484 & 0.889 
% \\
% \bottomrule
% \end{tabular}
% }
% \caption{
% \textbf{Multi-scene depth and view synthesis results}, on \emph{ScanNet-Frontal}. The \emph{shared} column, \emph{Lat} denotes a single shared latent space with per-scene decoders, \emph{Dec} denotes a single shared decoder with per-scene latent spaces, and \emph{All} denotes sharing both the latent space and the decoder. Interestingly, we notice marginal degradation in performance when using scene-specific latent spaces with a single shared decoder. Using a shared latent space, with scene-specific decoders, leads to further degradation in performance. Moreover, depth estimation results are more robust to multi-scene generalization than view synthesis. 
% }
% \label{table:nmvs_generalization}
% % \vspace{-4mm}
% \end{table*}





% % \captionsetup[table]{skip=6pt}

% % \begin{table*}[t!]
% % \small
% % \renewcommand{\arraystretch}{0.95}
% % \centering
% % {
% % \small
% % \setlength{\tabcolsep}{0.3em}
% % \begin{tabular}{l|c|c|c|c||c|c|c|c||c|c}
% % \toprule
% % \multirow{2}[2]{*}{\textbf{Version}} & 
% % \multirow{2}[2]{*}{\rotatebox{90}{\scriptsize{Self-Sup.}}} & \multirow{2}[2]{*}{\rotatebox{90}{\scriptsize{Shared}}} & \multirow{2}[2]{*}{\rotatebox{90}{\scriptsize{Decoder}}} & \multirow{2}[2]{*}{\rotatebox{90}{\scriptsize{\# Queries}}} & \multicolumn{4}{c||}{\textbf{Depth}} &
% % \multicolumn{2}{c}{\textbf{View Synthesis}}
% % \\
% % \cmidrule(lr){6-9} \cmidrule(lr){10-11} 
% % \renewcommand{\arraystretch}{1.0}
% % & & & & &
% % Abs.Rel.$\downarrow$ &
% % Sq.Rel.$\downarrow$ &
% % RMSE$\downarrow$ &
% % $\delta < {1.25}$$\uparrow$ &
% % PSNR$\uparrow$ & 
% % SSIM$\uparrow$
% % \\
% % %
% % \midrule
% % \rowcolor{Gray}
% % Volumetric & \checkmark & & V & $128$  
% % & 0.056 & 0.017 & 0.134 & 0.966 & 28.671 & 0.912 
% % \\
% % & & & V & $128$  
% % & 0.054 & 0.014 & 0.131 & 0.971 & 29.279 & 0.927 
% % \\
% % % \multirow{-2}{*}{Distilled (V $\shortrightarrow$ LD)} 
% % & \multirow{-3}{*}{\checkmark} & & LD & $1$  
% % % & 0.055 & 0.029 & 0.129 & 0.970 & 26.312 & 0.881 \\
% % & 0.057 & 0.029 & 0.139 & 0.962 & 27.663 & 0.901
% % % \\
% % % \rowcolor{Gray}
% % % & & & LD & $1$  
% % % % & 0.055 & 0.027 & 0.128 & 0.969 & 26.434 & 0.883 \\
% % % & 0.054 & 0.027 & 0.137 & 0.964 & 27.934 & 0.904 
% % \\
% % % \rowcolor{Gray}
% % % \multirow{-3}{*}{Refined (LD $\shortrightarrow$ V)} 
% % \multirow{-3}{*}{Distilled} 
% % & \multirow{-2}{*}{\checkmark} & & DL & $1\!\!+\!\!16$  
% % % & 0.054 & 0.029 & 0.127 & 0.971 & 29.331 & 0.912 \\
% % & 0.055 & 0.025 & 0.132 & 0.967 & 29.073 & 0.910 
% % \\
% % %
% % \midrule
% % \rowcolor{Gray}
% % Volumetric & \checkmark & L & V & $128$  
% % & 0.059 & 0.018 & 0.145 & 0.956 & 28.448 & 0.904 
% % \\
% % & & & V & $128$  
% % & -.---- & -.---- & -.---- & -.---- & -.---- & -.---- 
% % \\
% % \multirow{-2}{*}{Distilled (V $\shortrightarrow$ LD)} 
% % & \multirow{-2}{*}{\checkmark} & \multirow{-2}{*}{L} & LD & $1$  
% % & -.---- & -.---- & -.---- & -.---- & -.---- & -.---- 
% % \\
% % \rowcolor{Gray}
% % & & & LD & $1$  
% % & -.---- & -.---- & -.---- & -.---- & -.---- & -.---- 
% % \\
% % \rowcolor{Gray}
% % \multirow{-2}{*}{Guided (LD $\shortrightarrow$ V)} 
% % & \multirow{-2}{*}{\checkmark} & \multirow{-2}{*}{L} & LD+V & $1\!\!+\!\!16$  
% % & -.---- & -.---- & -.---- & -.---- & -.---- & -.---- 
% % \\
% % %
% % \midrule
% % \rowcolor{Gray}
% % Volumetric & \checkmark & D & V & $128$  
% % & 0.057 & 0.016 & 0.143 & 0.962 & 29.188 & 0.914 
% % \\
% % \rowcolor{White}
% % & & & V & $128$  
% % & 0.056 & 0.017 & 0.141 & 0.964 & 29.043 & 0.906 
% % \\
% % \multirow{-2}{*}{Distilled (V $\shortrightarrow$ LD)} 
% % & \multirow{-2}{*}{\checkmark} & \multirow{-2}{*}{D} & LD & $1$  
% % % & 0.055 & 0.034 & 0.138 & 0.968 & 26.084 & 0.879 \\
% % & 0.060 & 0.034 & 0.143 & 0.961 & 26.084 & 0.879 
% % \\
% % \rowcolor{Gray}
% % Distilled (V $\shortrightarrow$ LD, frozen)
% % & \checkmark & D & LD & $1$  
% % % & 0.055 & 0.028 & 0.135 & 0.968 & 26.101 & 0.880 \\
% % & 0.062 & 0.041 & 0.147 & 0.957 & 25.218 & 0.839 
% % \\
% % \rowcolor{White}
% % & & & LD & $1$  
% % % & 0.055 & 0.028 & 0.135 & 0.968 & 26.101 & 0.880 \\
% % & 0.058 & 0.028 & 0.135 & 0.963 & 26.101 & 0.880 
% % \\
% % \rowcolor{White}
% % \multirow{-2}{*}{Guided (LD $\shortrightarrow$ V)} 
% % & \multirow{-2}{*}{\checkmark} & \multirow{-2}{*}{D} & LD+V & $1\!\!+\!\!16$  
% % % & 0.055 & 0.031 & 0.133 & 0.969 & 28.355 & 0.905 \\
% % & 0.057 & 0.026 & 0.136 & 0.964 & 28.565 & 0.905 
% % \\
% % \bottomrule
% % \end{tabular}
% % }
% % \caption{
% % \textbf{Multi-scene depth and view synthesis results}, on \emph{ScanNet-Frontal}. The \emph{self-sup.} column denotes the use of the self-supervised photometric objective (\Section \ref{sec:photometric_loss}) as an additional source of regularization. In the \emph{shared} column, \emph{D} denotes a single shared decoder with per-scene latent spaces, and \emph{L} denotes a single shared latent space with per-scene decoders. In the \emph{decoder} column, \emph{V} denotes outputs from the volumetric head, and \emph{LD} denotes outputs from the light and depth field heads. The \emph{\# queries} column indicates the number of queries required for pixel rendering. 
% % }
% % \label{table:nmvs_ablation}
% % % \vspace{-4mm}
% % \end{table*}




==> tables/nmvs_view2.tex <==
\captionsetup[table]{skip=6pt}

\begin{table}[t!]
% \small
\renewcommand{\arraystretch}{0.9}
\centering
{
\small
\setlength{\tabcolsep}{0.25em}
\begin{tabular}{lc|cc}
\toprule
\textbf{Method} & &
PSNR & SSIM \\
\toprule
\multicolumn{2}{l|}{NSVF~\cite{liu2020neural}}
& $23.36$ & $0.823$ 
\\
\multicolumn{2}{l|}{SVS~\cite{Riegler2021SVS}}        
& $21.39$ & $\underline{0.914}$ 
\\
\multicolumn{2}{l|}{NeRF~\cite{mildenhall2020nerf}}
& $18.75$ & $0.751$ 
\\
\multicolumn{2}{l|}{NerfingMVS~\cite{nerfingmvs}}
& $22.10$ & $0.880$ 
\\
\midrule
\multirow{0}[2]{*}{\textbf{\Acronym}}
& R & $\textbf{25.88}$ & $\textbf{0.919}$ 
\\
& L & $\underline{25.34}$ & $0.907$ 
\\
\bottomrule
\end{tabular}
}
\caption{
\textbf{Per-scene view synthesis results}, on \emph{ScanNet-Frontal}. \Acronym improves view synthesis results (PSNR) in all considered scenes ($+9.8\% \pm 4.1\%$), relative to the previous state of the art~\cite{nerfingmvs}. Following \cite{wang2022r2l}, our method uses a deeper residual network for light field decoding to generate results comparable to---or even better than---volumetric rendering, whilst requiring a single network forward pass. 
}
\label{table:view_frontal}
\vspace{-2mm}
\end{table}

